Awareness of Secure Coding Guidelines in the Industry -- A first data analysis

Software needs to be secure, in particular, when deployed to critical infrastructures. Secure coding guidelines capture practices in industrial software engineering to ensure the security of code. This study aims to assess the level of awareness of secure coding in industrial software engineering, the skills of software developers to spot weaknesses in software code, avoid them, and the organizational support to adhere to coding guidelines. The approach draws on well-established theories of policy compliance, neutralization theory, and security-related stress and the authors' many years of experience in industrial software engineering and on lessons identified from training secure coding in the industry. The paper presents the questionnaire design for the online survey and the first analysis of data from the pilot study.

==> tables/tbl_q_summary.tex <==
\begin{spacing}{.7}
  \begin{table*}[http]
    \footnotesize
    \centering
    \begin{tabular}{p{4.6cm}|p{1.75cm}|p{4.8cm}|p{1.7cm}|}
      %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
      \cline{2-4}
      & \multicolumn{1}{|p{1.75cm}|}{\textbf{\# Questions}}
      & \textbf{~~~~~~~~~~~~~~~~~Constructs}
      & \textbf{~Reference} 
      \\ \hline
      %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
      %\multicolumn{1}{|p{4.6cm}|}{\textbf{General Questions}}
      %& ~~~~~~~~~9
      %& ~~~~~~~~~~~~~~~~~~~~~~~~~\textemdash
      %& ~~~~~~~\textemdash
      %\\ \hline
      %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
      \multicolumn{1}{|p{4.6cm}|}{\textbf{Policy Compliance (PC)}}
      & ~~~~~~~~~8
      & \begin{tabular}[c]{@{}l@{}}SE-C, ITC, GISA, ISPA,\\RespCost4, FacCond5\end{tabular}
      & \cite{bulgurcu2010information} \cite{moody2018toward}
      \\ \hline
      %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
      \multicolumn{1}{|p{4.6cm}|}{\textbf{Neutralization Theory (NT)}}
      & ~~~~~~~~~9
      & \begin{tabular}[l]{@{}l@{}}N-DON3, N-ATHL1, N-DOI1,\\N-DOR3, N-DOI2, N-DOI3,\\N-COC1, N-COC2, N-MOTL1\end{tabular}
      & \cite{siponen2010neutralization}
      \\ \hline
      %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
      \multicolumn{1}{|p{4.6cm}|}{\textbf{Security-Related-Stress (SRS)}}
      & ~~~~~~~~~6
      & CX2, CX4, OL1, OL4, UC1, UC4
      & \cite{d2014understanding}
      \\ \hline
    \end{tabular}
    \caption{Structure of the Survey Questions based on the the three Constructs (PC,NT,SRS)}
    \label{tab:survey:structure}
  \end{table*}
\end{spacing}
